Weakly But Deeply Supervised Occlusion-Reasoned Parametric Road Layouts

We propose an end-to-end network that takes a single perspective RGB image of a complex road scene as input, to produce occlusion-reasoned layouts in perspective space as well as a parametric bird's-eye-view (BEV) space. In contrast to prior works that require dense supervision such as semantic labels in perspective view, our method only requires human annotations for parametric attributes that are cheaper and less ambiguous to obtain. To solve this challenging task, our design is comprised of modules that incorporate inductive biases to learn occlusion-reasoning, geometric transformation and semantic abstraction, where each module may be supervised by appropriately transforming the parametric annotations. We demonstrate how our design choices and proposed deep supervision help achieve meaningful representations and accurate predictions. We validate our approach on two public datasets, KITTI and NuScenes, to achieve state-of-the-art results with considerably less human supervision.

==> tables/ablation_study.tex <==
\begin{tabular}{l|c|c|c|c|cccc}
  \hline
              &
              \multicolumn{4}{c|}{Module} &\multicolumn{4}{c}{KITTI~\cite{sam:Geiger13a}} \\
  \hline
  Method & \scriptsize{Perspective} & \scriptsize{Transformation} & \scriptsize{Hallucination} & \scriptsize{Parametric} &  Accu.-Bi. $\uparrow$ & Accu.-Mc. $\uparrow$ & MSE $\downarrow$ & F1 $\uparrow$ \\
  \hline
  RGB~\cite{sam:Seff16a} & & & & \checkmark& .811 & .778 & .230& .176\\
  \hline
  RGB+PS  & \checkmark & & & \checkmark & .822  & .827  & .159&  .425\\
  \hline
  RGB+PS+TS & \checkmark & \checkmark &  & \checkmark & .826 & .829 & .144 & 441 \\ 
  \hline
  Ours & \checkmark & \checkmark & \checkmark & \checkmark& .833 & .832 & .140 & .473 \\
  \hline
\end{tabular}

==> tables/attribute_definition.tex <==
\begin{tabular}{c|l|c}
  \hline
  Group & Attribute Definition & Prediction \\
  \hline
  \hline
  Binary $\Theta_{\textrm{b}}$ & Main road is curved or not & Binary \\
  & Main road is one-way or not & Binary \\
  & Main road delimiter existence & Binary \\
  & Delimiter between main road and sidewalk & Binary \\
  & Existence of left sidewalk & Binary \\
  & Existence of right sidewalk & Binary \\
  & Existence of crosswalk before intersection & Binary \\
  & Existence of crosswalk after intersection & Binary \\
  & Existence of crosswalk on the left side-road & Binary \\
  & Existence of crosswalk on the right side-road & Binary \\
  & Existence of crosswalk on the main road (no intersection) & Binary \\
  & Existence of left side-road & Binary \\
  & Existence of right side-road & Binary \\
  & Main road ends the side-road & Binary \\
  \hline
  Multiclass $\Theta_{\textrm{m}}$ & Number of lanes on the right of ego car & 0-11 \\
  & Number of lanes on the left of ego car & 0-11 \\
  \hline
  Continuous $\Theta_{\textrm{c}}$ & Main road rotation &  -1/8$~\pi$ - 1/8$~\pi$ \\
  & Width of left side-road & 0-30 m \\
  & Width of right side-road & 0-30 m \\
  & Main road delimiter width & 0-10 m \\
  & Starting point of left side-road & 0-60 m \\
  & Starting point of right side-road & 0-60 m \\
  & Distance to crosswalk on the main road & 0-60 m \\
  & Main road sidewalk width & 0-10 m\\
  & Main road sidewalk delimiter width & 0-10 m \\
  & Main road curvature & 1-Inf \\
  \hline
\end{tabular}


%    # #0:is_curve
%    # #1:is_oneway
%    # #2:delimiter_main
%    # #3:delimiter_sidewalk
%    # #4-5: sidewalk types:
%    #   #4:sidewalk exists on left
%    #   #5:sidewalk exists on right
%    # #6-10 cross walk types:
%    #   #6:cw_before
%    #   #7:cw_after
%    #   #8:cw_left
%    #   #9:cw_right
%    #   #10 cross walk on main street
%    # #11-12 road topology:
%    #   #11:has left side street
%    #   #12:has right side street
%    # #13 main road ends after sideroads

==> tables/intermediate_results.tex <==
\begin{tabular}{l|cc|ccccc|c}
  \hline
  &\multicolumn{2}{c|}{Representation} 
  &\multicolumn{6}{c}{KITTI~\cite{sam:Geiger13a}} \\
  \hline
  Method & Perspective & BEV & Road & Land Boundary & Sidewalk &  Crosswalk & Background & Average \\
  \hline
  RGB+PS  & \checkmark & & .689 & .365 & .226 & .010 & .954 & .449 \\
  \hline
  Ours  & \checkmark & & .700 & .403 & .255 & .042 & .962 & .472 \\
  & & \checkmark & .605 & .272 & .167 & .038 & .868 & .390 \\
  \hline
\end{tabular}

==> tables/intermediate_results_IOU.tex <==
\begin{tabular}{l|cc|ccccc|c}
  \hline
  &\multicolumn{2}{c|}{Representation} 
  &\multicolumn{6}{c}{KITTI~\cite{sam:Geiger13a}} \\
  \hline
  Method & Perspective & BEV & Road & Land Boundary & Sidewalk &  Crosswalk & Background & Average \\
  \hline
  RGB+PS & \checkmark & & .563 & .214 & .126 & .007 & .878 & .358 \\
  \hline
  Ours & \checkmark & & .605 &  .272 & .147 & .033  & .883 & .388 \\
  & & \checkmark & .461 & .197 & .102 & .032 & .651 & .289 \\
  \hline
\end{tabular}

==> tables/nuscenes_results.tex <==
\begin{tabular}{l|ccc}
  \hline
              & \multicolumn{3}{c}{NuScenes} \\
  \hline
  Method      & Accu.-Bi. $\uparrow$ &  Accu.-Mc. $\uparrow$ & MSE $\downarrow$ \\
  \hline
  RGB~\cite{sam:Seff16a,he2016deep} & .850 & .503 & .084 \\
  \hline
  BEV~\cite{Wang_2019_CVPR} & .846 & .485 & .073\\
  H-BEV+DA~\cite{Wang_2019_CVPR}+GM & .877 & .496 & .032\\
  \hline
  BEV-J-O~\cite{Liu_2020_CVPR}  & .858      & .543      & .027\\  
  \hline
  Ours & .875 & .560 & .023 \\    
  \hline
\end{tabular}

==> tables/statistics_obj_straight.tex <==
\begin{tabular}{l|ccccccccc|c}
\hline
  Obj. & 0 & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & Avg. \\
  \hline
  %&\multicolumn{10}{c}{Considering Four Semantic Classes} \\
  [16]  & .67 & .78 & .67 & .64 & .61 & .45 & .48 & .37 & .35 & .45\\
  Ours  & .78 & .81 & .72 & .69 & .67 & .48 & .50 & .40 & .35 & .50\\
  \hline
  IoU &\multicolumn{10}{c}{Considering Road Class Only} \\
  \hline
  [16]  & .85 & .74 & .85 & .79 & .67 & .63 & .59 & .57 & .37 & .63\\
  Ours  & .86 & .91 & .86 & .83 & .70 & .70 & .61 & .61 & .50 & .70\\
  \hline
  
\end{tabular}
